Strong Bisimulation for Control Operators

The purpose of this paper is to identify programs with control operators whose reduction semantics are in exact correspondence. This is achieved by introducing a relation $\simeq$, defined over a revised presentation of Parigot's $\lambda\mu$-calculus we dub $\Lambda M$. Our result builds on two fundamental ingredients: (1) factorization of $\lambda\mu$-reduction into multiplicative and exponential steps by means of explicit term operators of $\Lambda M$, and (2) translation of $\Lambda M$-terms into Laurent's polarized proof-nets (PPN) such that cut-elimination in PPN simulates our calculus. Our proposed relation $\simeq$ is shown to characterize structural equivalence in PPN. Most notably, $\simeq$ is shown to be a strong bisimulation with respect to reduction in $\Lambda M$, i.e. two $\simeq$-equivalent terms have the exact same reduction semantics, a result which fails for Regnier's $\sigma$-equivalence in $\lambda$-calculus as well as for Laurent's $\sigma$-equivalence in $\lambda\mu$.

==> macros.tex <==
%\usepackage[english]{babel}

\RequirePackage{silence}
\WarningFilter{remreset}{The remreset package}

%\let\proof\relax
%\let\endproof\relax
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{anyfontsize}
\usepackage{array}
\usepackage{bm}
\usepackage{booktabs}
\usepackage{cancel}
\usepackage{dashbox}
%\usepackage{enumitem}
\usepackage{etoolbox}
\usepackage{graphicx}
\usepackage{hyperref}
\usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{multirow}
\usepackage{prooftree}
%\usepackage{regnier-proofnets}
\usepackage{stmaryrd}
\SetSymbolFont{stmry}{bold}{U}{stmry}{m}{n}
%\usepackage{thmtools}
%\usepackage{thm-restate}
\usepackage{tikz}
\usetikzlibrary{arrows}
\usetikzlibrary{calc}
\usetikzlibrary{cd}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{decorations.markings}
\usepackage[normalem]{ulem}
\usepackage{xcolor}
\usepackage{xspace}
\usepackage{longtable}
\usepackage{appendix}
\setcounter{toappendix}{2}
\capturecounter{theorem}
%\capturecounter{figure}
\usepackage{wrapfig}


%%%% Conditional compilation for technical report vs. short paper
\newbool{compilePaper}

\newcommand{\ispaper}[2]{\ifbool{compilePaper}{#1}{#2}}


\newcommand{\partitle}[1]{\medskip\noindent{\textsf{\textbf{#1}}}}


%%%% Colored substitutions
\newbool{coloredSubstitutions}
\booltrue{coloredSubstitutions}  %% true=colorear; false=no colorear
%\boolfalse{coloredSubstitutions}  %% true=colorear; false=no colorear

\newlength{\itemwidth}

%\newcommand{\delia}[1]{\textcolor{blue} {#1}}
%\newcommand{\cdelia}[2]{\delia{{#2}}}
%\newcommand{\odelia}[1]{{\color{blue}\sout{#1}}}
%\newcommand{\deliaso}[2]{\delia{\sout{#1}{#2}}}
%\newcommand{\andres}[1]{\textcolor{red} {#1}}
%\newcommand{\oandres}[1]{{\color{red}\sout{#1}}}
%\newcommand{\candres}[2]{\textcolor{red} {#2}}
%\newcommand{\edu}[1]{\textcolor{magenta} {#1}}
%\newcommand{\oedu}[1]{{\color{magenta}\sout{#1}}}
%%% \newcommand{\edur}[2]{\edu{\cancel{#1}{#2}}}
%%% \newcommand{\eduso}[2]{\edu{\sout{#1}{#2}}}
%%% \newcommand{\cedu}[2]{\textcolor{magenta} {#2}}
%\newenvironment{edue}{
  %\medskip
    %\bgroup\color{magenta}
%}{
%\egroup
  %\medskip
%}
%%% \newenvironment{deliae}{\par\color{blue}\begin{tabular}{p{0.9\textwidth}}
%%%     \\}{\\\\
%%%     \end{tabular}\par}


%%%% Colored substitutions
\definecolor{replacementColor}{rgb}{1,0.5,0}
\definecolor{explicitReplacementColor}{rgb}{0,0.5,1}
\definecolor{explicitRenaming}{rgb}{0.5,0.5,0}
\definecolor{explicitSubstitution}{rgb}{0.5,0.7,1}
\definecolor{substitution}{rgb}{1,0.7,0.5}
\definecolor{replacementColorLMSC}{rgb}{0.8,0.12,0.5}


\theoremstyle{definition}
%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{lemma}{Lemma}
%\newtheorem{proposition}{Proposition}
%\newtheorem{remark}{Remark}


\newcommand{\Eg}{{\em E.g.~}}
\newcommand{\eg}{{\em e.g.~}}
\newcommand{\ie}{{\em i.e.~}}
\newcommand{\cf}{{\em cf.~}}

\newcommand{\coloneq}{\ensuremath{:=}}
\newcommand{\Coloneq}{\ensuremath{::=}}
\newcommand{\dbckslash}{\ensuremath{\setminus\!\!\setminus}}
\newcommand{\dslash}{\ensuremath{/\!\!/}}
\newcommand{\dbslash}{\ensuremath{\backslash\!\!\backslash}}
\newcommand{\llbrace}{\{\!\!\{}
\newcommand{\rrbrace}{\}\!\!\}}
%\newcommand{\llbracket}{[\![}
%\newcommand{\rrbracket}{]\!]}
%\newcommand{\llangle}{\langle\!\langle}
\newcommand{\llangle}{\langle\mkern-\thickmuskip\langle}
\newcommand{\rrangle}{\rangle\mkern-\thickmuskip\rangle}
\newcommand{\eqdef}{\mathrel{\raisebox{-1pt}{\ensuremath{\stackrel{\textit{\tiny{def}}}{=}}}}}
\newcommand{\eqalpha}{\ensuremath{=_{\alpha}}}
\newcommand{\eqregnier}{\ensuremath{\simeq_{\rsigma}}}
\newcommand{\eqlaurent}{\ensuremath{\simeq_{\lsigma}}}
%\newcommand{\eqsigma}{\ensuremath{\simeq_{\Sigma}}}
\newcommand{\eqsigmaer}{\ensuremath{\simeq_{\exren}}}
\newcommand{\emphdef}[1]{\textbf{\emph{#1}}}

\renewcommand{\l}{\ensuremath{\lambda}}

\newcommand{\A}{\ensuremath{\mathcal{A}}}
\newcommand{\C}{\ensuremath{\mathcal{C}}}
\newcommand{\I}{\ensuremath{\mathcal{I}}}
\renewcommand{\L}{\ensuremath{\mathcal{L}}}
\newcommand{\M}{\ensuremath{\mathcal{M}}}
\newcommand{\N}{\ensuremath{\mathcal{N}}}
\newcommand{\R}{\ensuremath{\mathcal{R}}}
\newcommand{\U}{\ensuremath{\mathcal{U}}}
\newcommand{\V}{\ensuremath{\mathcal{V}}}
\newcommand{\W}{\ensuremath{\mathcal{W}}}
\newcommand{\WN}[1]{\ensuremath{\mathcal{W\!N}_{#1}}}

\newcommand{\LM}{\ensuremath{\Lambda M^{\bullet}}}
\newcommand{\LMfull}{\ensuremath{\Lambda M}}
%\newcommand{\LM}{\ensuremath{LM}}
\newcommand{\lm}{\ensuremath{\lambda\mu}}
\newcommand{\lmsc}{\ensuremath{\lambda\mu^{s,c}}}

\newcommand{\SysW}{\ensuremath{\mathcal{W}_{\lambda\mu}}}
\newcommand{\SysWes}{\ensuremath{\mathcal{W}_{\lambda\mu}^{\mathtt{sh}}}}

\newcommand{\CR}{\ensuremath{\mathtt{CR}}}
\newcommand{\ctxt}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\ctxtSort}[2]{\ensuremath{\mathtt{#1}_{\mathsf{#2}}}}
\newcommand{\ctxtset}[1]{\ensuremath{\mathcal{#1}}}

\newcommand{\pos}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\posset}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\posupd}[3]{\ensuremath{{#1}^{#2}_{#3}}}
\newcommand{\mtp}[2]{\ensuremath{\mathsf{mtp}_{#2}({#1})}}

\newcommand{\lammu}{\ensuremath{\lambda\mu}}
\newcommand{\lscmu}{\ensuremath{\mathit{LSC}_{\lammu}}}
\newcommand{\Command}{\ensuremath{\mathcal{C}}}
\newcommand{\CommandES}{\ensuremath{\mathcal{C}_{\mathtt{e}}}}
\newcommand{\objects}[1]{\ensuremath{\mathcal{O}(#1)}}
\newcommand{\terms}[1]{\ensuremath{\mathcal{T}(#1)}}
\newcommand{\commands}[1]{\ensuremath{\mathcal{C}(#1)}}
\newcommand{\ObjectES}{\ensuremath{\mathcal{O}_{\mathtt{e}}}}
\newcommand{\Term}{\ensuremath{\mathcal{T}}}
\newcommand{\TermES}{\ensuremath{\mathcal{T}_{\mathtt{e}}}}
%\newcommand{\TermContext}{\ensuremath{\mathcal{C}}}
%\newcommand{\TermExplicit}{\ensuremath{\mathcal{T}_{\mathtt{e}}}}
\newcommand{\TermName}{\ensuremath{\mathcal{N}}}
%\newcommand{\TermValue}{\ensuremath{\mathcal{T}_{\mathtt{v}}}}
\newcommand{\TermVariable}{\ensuremath{\mathcal{V}}}

\newcommand{\Type}{\ensuremath{\mathcal{T}_\tau}}
\newcommand{\TypeMultiset}{\ensuremath{\mathcal{M}}}
\newcommand{\TypeVariable}{\ensuremath{\mathcal{B}}}

\newcommand{\Answer}{\ensuremath{\mathtt{A}}}

\newcommand{\exsubs}[2]{\ensuremath{
            \ifbool{coloredSubstitutions}
      {{\color{explicitSubstitution}{\bm{[}}}}
      {[}
      {#1}\backslash{#2}
            \ifbool{coloredSubstitutions}
      {{\color{explicitSubstitution}{\bm{]}}}}
      {]}
}
}
\newcommand{\exrepl}[3]{\ensuremath{
      \ifbool{coloredSubstitutions}
      {{\color{explicitReplacementColor}{\llbracket}}}
      {\llbracket}
    {#2}
    \backslash_{#1}{#3}
        \ifbool{coloredSubstitutions}
      {{\color{explicitReplacementColor}{\rrbracket}}}
      {\rrbracket}
}}


\newcommand{\exreplren}[3]{\lceil #1 \mid #2, #3 \rceil}

\newcommand{\termapp}[2]{\ensuremath{{#1}\,{#2}}}
\newcommand{\termabs}[2]{\ensuremath{\lambda{#1}.{#2}}}
\newcommand{\termcont}[2]{\ensuremath{\mu{#1}.{#2}}}
\newcommand{\termemst}{\ensuremath{\#}}
\newcommand{\termname}[2]{\ensuremath{[{#1}]\,{#2}}}
\newcommand{\termpush}[2]{\ensuremath{{#1}\cdot{#2}}}
\newcommand{\termsubs}[3]{\ensuremath{{#3}\exsubs{#1}{#2}}}
\newcommand{\termrepl}[4]{\ensuremath{{#4}\exrepl{#1}{#2}{#3}}}
\newcommand{\termconc}[2]{\ensuremath{{#1}::{#2}}}

%\newcommand{\singleterm}[1]{\ensuremath{\left[{#1}\right]}}
%\newcommand{\singleterm}[1]{\ensuremath{[{#1}]}}
%\newcommand{\mulstiterm}[2]{\ensuremath{\singleterm{#1}_{#2}}}
%\newcommand{\labelled}[2]{\ensuremath{{#1}^{#2}}}
%\newcommand{\lvarterm}[2]{\ensuremath{{#1}^{#2}}}
%\newcommand{\lappterm}[3]{\ensuremath{{#1}\mathrel{@_{#3}}{#2}}}
%\newcommand{\TMultiset}{\ensuremath{\mathcal{T}}}

\newcommand{\typeand}[3]{\ensuremath{{#1}\mathrel{\land_{#3}}{#2}}}
\newcommand{\typebase}{\ensuremath{\iota}}
\newcommand{\typechoice}[1]{\ensuremath{{#1}^{\ast}}}
\newcommand{\typecmd}{\ensuremath{\bot}}
\newcommand{\typeemst}{\ensuremath{\epsilon}}
\newcommand{\typefunc}[2]{\ensuremath{{#1}\to{#2}}}
\newcommand{\typeinter}[2]{\ensuremath{\lbrack{#1}\rbrack_{#2}}}
\newcommand{\typeor}[3]{\ensuremath{{#1}\mathrel{\lor_{#3}}{#2}}}
\newcommand{\typepush}[2]{\ensuremath{{#1}\cdot{#2}}}
\newcommand{\typeunion}[2]{\ensuremath{\langle{#1}\rangle_{#2}}}
\newcommand{\typeval}{\ensuremath{\mathtt{a}}}
\newcommand{\type}{T}
\newcommand{\emst}{\termemst}
\newcommand{\temst}{\typeemst}
\newcommand{\tconc}{\termconc{\!}{\!}}
\newcommand{\push}[2]{\typepush{#1}{#2}}

\newlength{\PNdist}
\setlength{\PNdist}{20pt}
\newlength{\PNmarg}
\setlength{\PNmarg}{10pt}
\newlength{\PNsize}
\setlength{\PNsize}{15pt}
\tikzstyle{PNcir}=[circle,draw=black,inner sep=0pt,text width=\PNsize]
\tikzstyle{PNsub}=[rectangle,draw=black,inner sep=5pt,minimum height=\PNsize,rounded corners=8pt]
%\tikzstyle{PNbox}=[rectangle,draw=black,inner sep=0pt,minimum height=\PNdist+\PNsize+\PNmarg,dashed]
\newcommand{\PNnode}[3][]{
\node[PNcir] (#2) [#1] {};
\node[#1] {#3}
}
\tikzstyle{PNardot}=[dashed,rounded corners=8pt]
\tikzstyle{PNarrow}=[rounded corners=8pt]
\tikzstyle{PNarout}=[-{triangle 45},rounded corners=8pt]
\tikzstyle{PNarold}=[-{open triangle 45},rounded corners=8pt]

\newcommand{\framenode}[2]{\framebox[#1][c]{\parbox{#1}{\centering #2}}}
\newcommand{\dashnode}[2]{\dashbox[#1][c]{\parbox{#1}{\centering #2}}}

\newcommand{\topn}[1]{\ensuremath{#1^\lozenge}}
\newcommand{\topnd}[1]{\ensuremath{{#1}^{\blacklozenge}}}

\newcommand{\toform}[1]{\ensuremath{{#1}^\diamond}}

\newcommand{\formbase}{\ensuremath{\iota}}
\newcommand{\formbang}[1]{\ensuremath{{!}{#1}}}
\newcommand{\formder}[1]{\ensuremath{{?}{#1}}}
\newcommand{\formneg}[1]{\ensuremath{{#1}^\bot}}
\newcommand{\formpar}[2]{\ensuremath{{#1}\mathbin{\nomformpar}{#2}}}
\newcommand{\nomformpar}{\ensuremath{\mathbin{\bindnasrepma}}}
\newcommand{\formten}[2]{\ensuremath{{#1}\nomformten{#2}}}
\newcommand{\nomformten}{\ensuremath{\otimes}}

\newcommand{\sequ}[3]{\ensuremath{{#1}\vdash{#2}\mid{#3}}}
\newcommand{\sequM}[3]{\ensuremath{{#1}\vdash{#2}\mid{#3}}}
\newcommand{\assign}[2]{\ensuremath{{#1}:{#2}}}
\newcommand{\derivable}[3]{\ensuremath{{#1}\rhd_{#3}{#2}}}
\newcommand{\derivation}[5]{\ensuremath{{#1}_{\sequ{#2}{\assign{#3}{#4}}{#5}}}}

\newcommand{\ctxtand}[3]{\ensuremath{{#1}\mathrel{\land_{#3}}{#2}}}
\newcommand{\ctxtapp}[2]{\ensuremath{{#1}\langle{#2}\rangle}}
\newcommand{\ctxtor}[3]{\ensuremath{{#1}\mathrel{\lor_{#3}}{#2}}}
\newcommand{\ctxtres}[3]{\ensuremath{{#1}\mathrel{\dbckslash_{#3}}{#2}}}
\newcommand{\ctxtsum}[3]{\ensuremath{{#1}\mathrel{+_{#3}}{#2}}}
\newcommand{\ctxtwoc}[2]{\ensuremath{{#1}\llangle{#2}\rrangle}}

\newcommand{\ctxtLTT}{\ctxt{LTT}}
\newcommand{\ctxtLTC}{\ctxt{LTC}}
\newcommand{\ctxtLCC}{\ctxt{LCC}}
\newcommand{\ctxtLCT}{\ctxt{LCT}}

%\newcommand{\merge}[1]{\ensuremath{\mathsf{merge}\!({#1})}}
%\newcommand{\erase}[1]{\ensuremath{\mathsf{erase}({#1})}}
%\newcommand{\erase}[1]{\ensuremath{|{#1}|}}

\newcommand{\dom}[1]{\ensuremath{\mathtt{dom}({#1})}}

\newcommand{\applyax}[2]{\ensuremath{\mathtt{AX}({#1},{#2})}}
\newcommand{\applyval}[2]{\ensuremath{\mathtt{VAL}({#1},{#2})}}
\newcommand{\applyabs}[2]{\ensuremath{\mathtt{ABS}({#1},{#2})}}
\newcommand{\applyapp}[3]{\ensuremath{\mathtt{APP}({#1},{#2},{#3})}}

\newcommand{\projctxt}[1]{\ensuremath{\mathtt{CTXT}({#1})}}
\newcommand{\projprem}[1]{\ensuremath{\mathtt{PREM}({#1})}}
\newcommand{\projrule}[1]{\ensuremath{\mathtt{RULE}({#1})}}
\newcommand{\projsubj}[1]{\ensuremath{\mathtt{SUBJ}({#1})}}
\newcommand{\projtype}[1]{\ensuremath{\mathtt{TYPE}({#1})}}

\newcommand{\bn}[1]{\ensuremath{\mathtt{bn}({#1})}}
\newcommand{\bv}[1]{\ensuremath{\mathtt{bv}({#1})}}
\newcommand{\fn}[1]{\ensuremath{\mathtt{fn}({#1})}}
\newcommand{\fnp}[2]{\ensuremath{\mathtt{fn}_{#1}({#2})}}
\newcommand{\fnSort}[2]{\ensuremath{\mathtt{fn}_{\mathsf{#1}}({#2})}}
\newcommand{\fv}[1]{\ensuremath{\mathtt{fv}({#1})}}
\newcommand{\fvp}[2]{\ensuremath{\mathtt{fv}_{#1}({#2})}}
\newcommand{\fvSort}[2]{\ensuremath{\mathtt{fv}_{\mathsf{#1}}({#2})}}

\newcommand{\size}[1]{\ensuremath{\mathtt{sz}({#1})}}
\newcommand{\sz}[1]{\ensuremath{\mathtt{sz}({#1})}}
\newcommand{\struct}[1]{\ensuremath{\mathtt{st}({#1})}}

%\newcommand{\oc}[1]{\ensuremath{\mathtt{oc}({#1})}}  % conflict with
%tikz extension for PNs
\newcommand{\roc}[1]{\ensuremath{\mathtt{r}\oc{#1}}}
\newcommand{\toc}[1]{\ensuremath{\mathtt{TOC}({#1})}}
\newcommand{\troc}[1]{\ensuremath{\mathtt{TROC}({#1})}}

\newcommand{\residuals}[2]{\ensuremath{{#1}/{#2}}}

\newcommand{\prefix}{\ensuremath{\leq}}

\newcommand{\rrule}[1]{\ensuremath{\mathrel{\mapsto_{#1}}}}
\newcommand{\rewrite}[2][]{\ensuremath{\mathrel{\rightarrow^{#1}_{#2}}}}
\newcommand{\rewriten}[2][]{\ensuremath{\mathrel{\twoheadrightarrow^{#1}_{#2}}}}
\newcommand{\reduce}[1][]{\ensuremath{\mathrel{\rightsquigarrow^{#1}}}}

\newcommand{\reduction}[4]{\ensuremath{{#1}:{#2}\rewrite{#4}{#3}}}
\newcommand{\reductionn}[4]{\ensuremath{{#1}:{#2}\rewriten{#4}{#3}}}

\newcommand{\needed}{\ensuremath{\mathtt{nd}}}
\newcommand{\headnd}{\ensuremath{\mathtt{hnd}}}
\newcommand{\weaknd}{\ensuremath{\mathtt{whnd}}}

\newcommand{\callbyname}{\ensuremath{\mathtt{name}}}
\newcommand{\callbyneed}{\ensuremath{\mathtt{need}}}

\newcommand{\rB}{\ensuremath{\mathtt{B}}}
\newcommand{\rM}{\ensuremath{\mathtt{M}}}
\newcommand{\rS}{\ensuremath{\mathtt{S}}}
\newcommand{\rR}{\ensuremath{{\mathtt{R}^\bullet}}}
\newcommand{\rRlin}{\ensuremath{{\mathtt{R}^\circ}}}
\newcommand{\rRliner}{\ensuremath{{\mathtt{R}^\circ_{\tt er}}}}
\newcommand{\rRlinn}{\ensuremath{{\mathtt{R}^\circ_{{\tt n}}}}}
\newcommand{\rRfull}{\ensuremath{\mathtt{R}}}
\newcommand{\rC}{\ensuremath{\mathtt{C}}}
\newcommand{\rW}{\ensuremath{\mathtt{W}}}
%\newcommand{\rC}{\ensuremath{\mathtt{C}^\bullet}}

\newcommand{\BMnf}{\downarrow \rB\rM}
\newcommand{\BMform}{\rB\rM\mbox{-nf}}
%\newcommand{\Can}{\mathtt{can}} %canonical normal-form
\newcommand{\Can}{\mathfrak{C}} %canonical normal-form
\newcommand{\BMCnf}{\downarrow \Can}
\newcommand{\BMCform}{\Can\mbox{-nf}}
\newcommand{\BMCName}{\ensuremath{{\Can}}}
\newcommand{\BMC}[1]{\ensuremath{\Can({#1})}}
\newcommand{\BMName}{\ensuremath{{\mathsf{BM}}}}
\newcommand{\Cform}{\rC\mbox{-nf}}

\newcommand{\dB}{\ensuremath{\mathtt{dB}}}
\newcommand{\dU}{\ensuremath{\mathtt{dU}}}
\newcommand{\lsv}{\ensuremath{\mathtt{lsv}}}

%\newcommand{\hn}{\ensuremath{\mathtt{hnd}}}
%\newcommand{\whn}{\ensuremath{\mathtt{whn}}}
\newcommand{\alw}{\ensuremath{\mathtt{alw}}}
%\newcommand{\lbl}{\ensuremath{\mathtt{lbl}}}
%\newcommand{\rdx}{\ensuremath{\mathtt{rdx}}}

%\newcommand{\set}[1]{\ensuremath{\left\{{#1}\right\}}}
\newcommand{\set}[1]{\ensuremath{\{{#1}\}}}
\newcommand{\multiset}[1]{\ensuremath{\llbrace{#1}\rrbrace}}
\newcommand{\project}[1]{\ensuremath{{#1}^\downarrow}}
\newcommand{\projectSort}[2]{\ensuremath{{#2}_{\mathsf{#1}}^\downarrow}}
\newcommand{\iredos}[2]{\ensuremath{{
      \ifbool{coloredSubstitutions}
      {{\color{replacementColor}{\llbrace}}}
      {\llbrace}
      {#1}\backslash {#2}
      \ifbool{coloredSubstitutions}
      {{\color{replacementColor}{\rrbrace}}}
      {\rrbrace}
    }}}

\newcommand{\ire}[3]{\ensuremath{{
      \ifbool{coloredSubstitutions}
      {{\color{replacementColor}{\llbrace}}}
      {\llbrace}
      {#1}\backslash_{#2} {#3}
      \ifbool{coloredSubstitutions}
      {{\color{replacementColor}{\rrbrace}}}
      {\rrbrace}
}}}

\newcommand{\iremany}{\ensuremath{{
      \ifbool{coloredSubstitutions}
      {{\color{replacementColor}{\llbrace}}}
      {\llbrace}
      {\alpha_1}\backslash_{\alpha'_1} {u_1} \ldots
      {\alpha_n}\backslash_{\alpha'_n} {u_n}
      \ifbool{coloredSubstitutions}
      {{\color{replacementColor}{\rrbrace}}}
      {\rrbrace}
    }}}


\newcommand{\replace}[4]{\ensuremath{{{#4}
      \ifbool{coloredSubstitutions}
      {{\color{replacementColor}{\llbrace}}}
      {\llbrace}
      {#2}\backslash_{#1}{#3}
      \ifbool{coloredSubstitutions}
      {{\color{replacementColor}{\rrbrace}}}
      {\rrbrace}
}}}
\newcommand{\replaceo}[3]{\ensuremath{{
      \ifbool{coloredSubstitutions}
      {{\color{replacementColor}{\llbrace}}}
      {\llbrace}
      {#2}\backslash_{#1}{#3}
      \ifbool{coloredSubstitutions}
      {{\color{replacementColor}{\rrbrace}}}
      {\rrbrace}
    }}}
\newcommand{\replaceMulti}[4]{\ensuremath{{{#4}
      \overrightarrow{\ifbool{coloredSubstitutions}
      {{\color{replacementColor}{\llbrace}}}
      {\llbrace}
      {#2}\backslash_{#1}{#3}
      \ifbool{coloredSubstitutions}
      {{\color{replacementColor}{\rrbrace}}}
      {\rrbrace}
      }}}}

  \newcommand{\subsdos}[2]{\ensuremath{{
          \ifbool{coloredSubstitutions}
          {{\color{substitution}{\bm{\{}}}}
          {\{}
            {#1}\backslash{#2}
        \ifbool{coloredSubstitutions}
        {{\color{substitution}{\bm{\}}}}}
        {\}}
      }}}
  \newcommand{\substitute}[3]{\ensuremath{{{#3}
          \ifbool{coloredSubstitutions}
          {{\color{substitution}{\bm{\{}}}}
          {\{}
            {#1}\backslash{#2}
        \ifbool{coloredSubstitutions}
        {{\color{substitution}{\bm{\}}}}}
        {\}}
      }}}
  \newcommand{\substituteplus}[3]{\ensuremath{{{#3}
          \ifbool{coloredSubstitutions}
          {{\color{substitution}{\bm{\{}}}}
          {\{}
            {#1}\backslash{#2}
        \ifbool{coloredSubstitutions}
        {{\color{substitution}{\bm{\}}}}}
        {\}}
      }}}

%\newcommand{\substituteL}[4]{\ensuremath{{\llbrace{#2}/{#1}\rrbrace_{#3}{#4}}}}
\newcommand{\substituteT}[4]{\ensuremath{{{#3}\left\{{#1}/{#2}\right\}_{#4}}}}
\newcommand{\many}[2]{\ensuremath{({#1})_{#2}}}

\newcommand{\Rew}[1]{\rightarrow_{#1}}
\newcommand{\LRew}[1]{\; \! \mbox{}_{#1}{\leftarrow}\ }
\newcommand{\LRewn}[1]{\; \! {}_{#1}\twoheadleftarrow\ }
\newcommand{\Rewplus}[1]{\rightarrow^{+}_{#1}}
\newcommand{\Rewn}[1]{\twoheadrightarrow_{#1}}
\newcommand{\Rewnp}[2]{\twoheadrightarrow^{#1}_{#2}}

\newcommand{\NF}[1]{\ensuremath{\mathcal{N\!F}_{#1}}}
\newcommand{\HNF}[1]{\ensuremath{\mathcal{H}\NF{#1}}}
\newcommand{\WHNF}[1]{\ensuremath{\mathcal{W}\HNF{#1}}}
\newcommand{\ANF}{\ensuremath{\mathcal{ANF}}}

\newcommand{\nf}[2]{\ensuremath{\mathtt{nf}_{#1}({#2})}}
\newcommand{\hnf}[2]{\ensuremath{\mathtt{hnf}_{#1}({#2})}}
\newcommand{\whnf}[2]{\ensuremath{\mathtt{whnf}_{#1}({#2})}}
\newcommand{\anf}[1]{\ensuremath{\mathtt{ANF}({#1})}}

\newcommand{\BM}[1]{\ensuremath{\mathsf{BM}({#1})}}
\newcommand{\B}[1]{\ensuremath{\mathsf{B}({#1})}}
%\newcommand{\BMsort}[2]{\ensuremath{\mathsf{BM}_{\mathsf{#1}}({#2})}}
%\newcommand{\BMCsort}[2]{\ensuremath{\mathsf{BMC}_{\mathsf{#1}}({#2})}}

%\newcommand{\mcnf}[1]{\ensuremath{\mathsf{mcnf}\left({#1}\right)}}
\newcommand{\mcnf}[1]{\ensuremath{\topnd{\left({#1}\right)}}}

%\newcommand{\whnf}[1]{\ensuremath{\mathtt{W}\hnf{#1}}}
%\newcommand{\res}[2]{\ensuremath{\mathtt{res}({#1}/{#2})}}
%\newcommand{\pos}[1]{\ensuremath{\mathtt{pos}({#1})}}
\newcommand{\termat}[2]{\ensuremath{{#1}|_{#2}}}
\newcommand{\treeat}[2]{\ensuremath{{#1}|_{#2}}}
\newcommand{\replaceat}[3]{\ensuremath{{#1}[{#3}]_{#2}}}

\newcommand{\ruleName}[1]{\ensuremath{\mathtt{({#1})}}}
\newcommand{\ruleAndI}{\ruleName{\land i}}
%\newcommand{\ruleAndE}{\ruleName{\land e}}
\newcommand{\ruleArrowE}{\ruleName{\typefunc{\!}{\!}e}}
\newcommand{\ruleArrowI}{\ruleName{\typefunc{\!}{\!}i}}
\newcommand{\ruleAxiom}{\ruleName{ax}}
\newcommand{\ruleBottomE}{\ruleName{\typecmd e}}
\newcommand{\ruleBottomI}{\ruleName{\typecmd i}}
\newcommand{\ruleCut}{\ruleName{es}}
\newcommand{\ruleEqSubsSwap}{\ensuremath{\Sigma_{1}}}
\newcommand{\ruleEqSubsAbs}{\ensuremath{\Sigma_{2}}}
\newcommand{\ruleEqSubsApp}{\ensuremath{\Sigma_{3}}}
\newcommand{\ruleEqSubsCont}{\ensuremath{\Sigma_{4}}}
\newcommand{\ruleEqReplSwap}{\ensuremath{\Sigma_{5}}}
\newcommand{\ruleEqReplCont}{\ensuremath{\Sigma_{6}}}
\newcommand{\ruleEqReplH}{\ensuremath{\Sigma_{67}}}
\newcommand{\ruleEqReplContAbs}{\ensuremath{\Sigma_{7}}}
\newcommand{\rulelinearreplacement}{\ensuremath{\Sigma_{8}}}
\newcommand{\ruleEqPushPush}{\ensuremath{\Sigma_{9}}}
\newcommand{\ruleEqPushPop}{\ensuremath{\Sigma_{10}}}
\newcommand{\ruleEqPopPop}{\ensuremath{\Sigma_{11}}}
\newcommand{\ruleEqENamRepl}{\ensuremath{\Sigma_{12}}}
\newcommand{\ruleEqENamCont}{\ensuremath{\Sigma_{13}}}
\newcommand{\ruleEqENamAbs}{\ensuremath{\Sigma_{14}}}

\newcommand{\ruleValue}{\ruleName{val}}
%\newcommand{\ruleValueL}{\ruleName{val}}
%\newcommand{\ruleValueU}{\ruleName{valU}}
%\newcommand{\ruleMultiVar}{\ruleName{mVar}}
%\newcommand{\ruleMultiOmega}{\ruleName{m\omega}}
%\newcommand{\ruleMultiArrowE}{\ruleName{m\typefunc{\!}{\!}e}}
%\newcommand{\ruleMultiArrowI}{\ruleName{m\typefunc{\!}{\!}i}}
\newcommand{\Rule}[3]{
    \prooftree
         #1
    \justifies  
         #2
    \thickness=0.05em
    \using
         #3
    \endprooftree}

\newcommand{\equivst}{\approx}
\newcommand{\ih}{\ensuremath{\mathit{i.h.}}\xspace}

\newcommand{\rootpos}{\ensuremath{\epsilon}}
\newcommand{\emptyred}{\ensuremath{\mathit{nil}}}
\newcommand{\obs}[1]{\cong_{#1}}  %% defined in lmcs

\newcommand{\eren}[2]{
        \ifbool{coloredSubstitutions}
      {{\color{explicitRenaming}{\bm{[}}}}
      {[}
      {#1}
\backslash
{#2}
        \ifbool{coloredSubstitutions}
      {{\color{explicitRenaming}{\bm{]}}}}
      {]}
    }
    
\newcommand{\iren}[2]{\{ {#1}\backslash{#2}\} }

\newcommand{\freeFor}[2]{\ensuremath{\mathtt{fc}({#1},{#2})}}
\newcommand{\notfreev}[2]{#1 \notin \fv{#2}}
\newcommand{\notfreen}[2]{#1 \notin \fn{#2}}
\newcommand{\notatall}[2]{#1 \notin #2}

\newcommand{\muplus}{\mu^{s}}
\newcommand{\replaceplus}[4]{\ensuremath{{{#4}
      \ifbool{coloredSubstitutions}
      {{\color{replacementColorLMSC}{\llangle}}}
      {\llangle}
      % {#2}\triangleleft_{#1}{#3}
            {#2}\backslash_{#1}{#3}
      \ifbool{coloredSubstitutions}
      {{\color{replacementColorLMSC}{\rrangle}}}
      {\rrangle}
    }}}


\newcommand{\termsLM}{\ensuremath{{\cal T}}}
\newcommand{\commandsLM}{\ensuremath{{\cal K}}}
\newcommand{\objectsLM}{\ensuremath{{\cal O}}}
\newcommand{\pureObjectsLM}{\ensuremath{{\cal O}^p}}
\newcommand{\paral}{\Rightarrow}
\newcommand{\paralSort}[1]{\Rightarrow_{\mathsf{#1}}}

\newcommand{\ruleParVar}{\ruleName{PVar}}
\newcommand{\ruleParLam}{\ruleName{PLam}}
\newcommand{\ruleParApp}{\ruleName{PApp}}
\newcommand{\ruleParBeta}{\ruleName{PBeta}}
\newcommand{\ruleParCont}{\ruleName{PCont}}
\newcommand{\ruleParName}{\ruleName{PName}}
\newcommand{\ruleParRen}{\ruleName{PRen}}
\newcommand{\ruleParStackBase}{\ruleName{PStackBase}}
\newcommand{\ruleParStackInd}{\ruleName{PStackInd}}
\newcommand{\ruleParMu}{\ruleName{PMu}}
\newcommand{\rt}{\rho\theta}
\newcommand{\sig}{{\sigma}}
\newcommand{\ovsig}{\overline{\sigma}}
\long\def\ignore#1{\relax}
\newcommand{\renproj}[1]{#1^{\Downarrow}}
\newcommand{\BMR}[1]{\renproj{\BM{#1}}}
\newcommand{\lvec}[1]{\overrightarrow{#1}}
\newcommand{\exren}{{{\tt er}}}
\newcommand{\eqexsubs}{{\tt exs}}
\newcommand{\eqexrepl}{{\tt exr}}
\newcommand{\eqexren}{{\tt exren}}
\newcommand{\eqexrr}{{\tt exrr}}
\newcommand{\eqlinear}{{\tt lin}}
\newcommand{\eqpoppop}{{\tt pp}}
\newcommand{\eqrho}{\rho}
\newcommand{\eqtheta}{\theta}
\newcommand{\eqren}{{\tt ren}}

\newcommand{\regnier}{$\Sigma$\xspace}
\newcommand{\pair}[2]{\langle #1, #2 \rangle}

\newcommand{\defn}[1]{\textbf{#1}}
\newcommand{\stextbf}[1]{{\footnotesize \textbf{#1}}}
\newcommand{\Gam}{\Gamma}
\newcommand{\Del}{\Delta}
\newcommand{\tarrow}{\rightarrow}
\newcommand{\sep}{\hspace{.3cm}}

\newcommand{\tax}{{\tt ax}}
\newcommand{\app}{{\tt app}}
\newcommand{\absin}{{\tt abs}_{\in}}
\newcommand{\absnotin}{{\tt abs}_{\notin}}
\newcommand{\abs}{{\tt abs}}
\newcommand{\namein}{{\tt name}_{\in}}
\newcommand{\namenotin}{{\tt name}_{\notin}}
\newcommand{\nametr}{{\tt name}}
\newcommand{\subin}{{\tt sub}_{\in}}
\newcommand{\subnotin}{{\tt sub}_{\notin}}
\newcommand{\subtr}{{\tt sub}}
\newcommand{\muin}{{\mu}_{\in}}
\newcommand{\munotin}{{\mu}_{\notin}}
\newcommand{\mutr}{{\mu}}
\newcommand{\renin}{{\tt ren}_{\in}}
\newcommand{\rennotin}{{\tt ren}_{\notin}}
\newcommand{\ren}{{\tt ren}}
\newcommand{\treplin}{{\tt repl}_{\in}}
\newcommand{\treplnotin}{{\tt repl}_{\notin}}
\newcommand{\trepl}{{\tt repl}}
\newcommand{\stacku}{{\tt st}_h}
\newcommand{\stackd}{{\tt st}_t}
\newcommand{\lmu}{\lambda\mu}
\newcommand{\tradlaurentu}[1]{#1^\circ}
\newcommand{\tradlaurentd}[1]{#1^\bullet}
\newcommand{\dem}{\triangleright}
\newcommand{\tcut}{{\tt cut}}
\newcommand{\expansion}[1]{{\tt e}(#1)}
\newcommand{\deft}[1]{{\bf #1}}
\newcommand{\al}{\alpha}
\newcommand{\ga}{\gamma}
\newcommand{\Id}{{\tt I}}
\newcommand{\isubs}[2]{\substitute{#1}{#2}{}}
\newcommand{\esta}{\leq 1}
\newcommand{\redpn}{{\tt PPN}}
\newcommand{\neren}[2]{\exrepl{#2}{#1}{\termemst}}

\tikzset{negated/.style={
        decoration={markings,
            mark= at position 0.5 with {
                \node[transform shape] (tempnode) {$/$};
            }
        },
        postaction={decorate}
    }
}

%\newcommand{\rsigma}{R}
\newcommand{\rsigma}{\sigma}
%\newcommand{\lsigma}{L}
\newcommand{\lsigma}{\sigma}
% \newcommand{\esigma}{R^B}
\newcommand{\esigma}{\sigma^B}
%\newcommand{\elsigma}{L^B}
\newcommand{\elsigma}{\sigma^B}
\newcommand{\trad}[1]{{\tt F}(#1)}

\newcommand{\diagexuno}{\eqexsubs\mbox{-}1}
\newcommand{\diagexdos}{\eqexsubs\mbox{-}2}
\newcommand{\diagextres}{\eqexsubs\mbox{-}3}
\newcommand{\diageruno}{\eqexrepl\mbox{-}1}
\newcommand{\diagerdos}{\eqexrepl\mbox{-}2}
\newcommand{\diagertres}{\eqexrepl\mbox{-}3}
\newcommand{\diaglinuno}{\eqlinear\mbox{-}1}
\newcommand{\diaglindos}{\eqlinear\mbox{-}2}

\newcommand{\scaleinput}[2]{\scalebox{#1}{\input{#2}}}

\newcommand{\aax}{a}
\newcommand{\lpar}{\mathbin{\bindnasrepma}}
\newcommand{\bltimes}{\otimes}
\newcommand{\derel}{d}
\newcommand{\boxn}{b}
\newcommand{\weakn}{w}
\newcommand{\cont}{c}
\newcommand{\axcut}{{\tt C}(\aax)}
\newcommand{\multcut}{{\tt C}(\lpar,\bltimes)}
\newcommand{\derboxcut}{{\tt C}(\derel,\boxn)}
\newcommand{\weakboxcut}{{\tt C}(\weakn,\boxn)}
\newcommand{\boxboxcut}{{\tt C}(\boxn,\boxn)}
\newcommand{\contboxcut}{{\tt C}(\cont,\boxn)}
\newcommand{\weaktencut}{{\tt C}(\weakn,\bltimes)}
\newcommand{\conttencut}{{\tt C}(\cont,\bltimes)}
\newcommand{\boxtencut}{{\tt C}(\boxn,\bltimes)}
\newcommand{\rRstackvacio}{{\tt R}_{\termemst}}
\newcommand{\rRstacknovacio}{{\tt R}_{\neg\termemst }}
\newcommand{\rRdiffu}{{\tt R}_{\neg\termemst }^{\neq 1}}
\newcommand{\rRequ}{{\tt R}_{\neg\termemst }^{=1}}
% \newcommand{\rRswap}{{\tt R}_{\termemst, \neg\termemst  }^{=1}}
\newcommand{\rRswap}{{\tt swap}}
% \newcommand{\composition}{{\tt R}_{\neg\termemst,\neg\termemst }^{=1}}
\newcommand{\composition}{{\tt comp}}
% \newcommand{\nonlinrRswap}{{\tt R}_{\termemst, \neg\termemst }^{=1,{\tt nonlin}}}
\newcommand{\nonlinrRswap}{\rW_{\neg {\tt lin}}}
%\newcommand{\nonlincomposition}{{\tt R}_{\neg\termemst,\neg\termemst }^{=1,{\tt nonlin}}}
\newcommand{\nonlincomposition}{\rC_{\neg {\tt lin}}}
% \newcommand{\prelineal}{{\tt name\mbox{-}pre\mbox{-}lin}}
\newcommand{\prelineal}{{\tt name}}
% \newcommand{\nonprelineal}{{\tt name\mbox{-}nonlin}}
% \newcommand{\nonprelineal}{{\tt nonlin}}
\newcommand{\nonprelineal}{{\tt N}_{\neg {\tt lin}}}
% \newcommand{\lineal}{{\tt lin}}
\newcommand{\linealrule}{{\tt N}}
\newcommand{\lineal}{{\tt lin}}

\newcommand{\nest}[1]{\ensuremath{\mathbf{#1}}}
  
%%%Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> proof-replacement-bis.tex <==
\delia{Esta prueba asume que no hay restricciones de
  variables sobre los comandos}

\begin{proof} We reason by induction on $o$. 
  \begin{itemize}
    \item $o = x$. Then $\replace{\alpha'}{\alpha}{s}{x} = x$. The statement
    holds for $\Gam^* = \Gam$ and $\Del^*  = \emptyset$ and
    $(\al:S\tarrow B)^{\esta}$ equal to empty.
    
    \item $o = \termapp{t}{u}$. Then
    $\replace{\alpha'}{\alpha}{s}{(\termapp{t}{u})}  =
    \termapp{\replace{\alpha'}{\alpha}{s}{t}}{\replace{\alpha'}{\alpha}{s}{u}}$.
    This holds by the \ih
    
    \item $o= \termabs{x}{t}$. Then
    $\replace{\alpha'}{\alpha}{s}{(\termabs{x}{t})} =
    \termabs{x}{\replace{\alpha'}{\alpha}{s}{t}}$, where $x \notin \fv{s}$.
    This holds by the \ih
    
    \item $o =\termcont{\beta}{c}$. Then
    $\replace{\alpha'}{\alpha}{s}{(\termcont{\beta}{c})} =
    \termcont{\beta}{\replace{\alpha'}{\alpha}{s}{c}}$, where $\beta \notin
    \fn{s, \alpha, \al'}$. This holds by the \ih

    \item $o= \termsubs{x}{u}{t}$. Then
    $\replace{\alpha'}{\alpha}{s}{\termsubs{x}{u}{t}} =
    \termsubs{x}{\replace{\alpha'}{\alpha}{s}{u}}{\replace{\alpha'}{\alpha}{s}{t}}$,
    where $x \notin \fv{s}$. This holds by the \ih
    
    \item $o=\termname{\alpha}{t}$. Then
    $\replace{\alpha'}{\alpha}{s}{(\termname{\alpha}{t})} =
    \termname{\alpha'}{(\termconc{\replace{\alpha'}{\alpha}{s}{t}}{s})}$. The
    typing derivation for $o$ has the following form: \[
    \Rule{\Gam \vdash t:S \tarrow B \mid \Del, (\al: S \tarrow B)^{\leq 1}}
         {\Gam \vdash \termname{\alpha}{t} \mid \Del, \al: S \tarrow B}
         {} \]
    The \ih gives $\Gam^{**} \vdash \replace{\alpha'}{\alpha}{s}{t} : S
    \tarrow B \mid \Del^{**}$, where $\Gam^{**} \subseteq \Gam \cup \Gam'$ and
    $\Del^{**} \subseteq \Del  \cup \Del'\cup (\alpha':B)$.
    Lemma~\ref{l:application} gives $\Gam^{**} \cup \Gam' \vdash
    \termconc{\replace{\alpha'}{\alpha}{s}{t}}{s} :  B \mid \Del^{**} \cup
    \Del'$. Then we get $\Gam^{**} \cup \Gam' \vdash
    \termname{\al'}{\termconc{\replace{\alpha'}{\alpha}{s}{t}}{s}} \mid
    \Del^{**} \cup \Del', \al' : B$ by rule $(\nametr)$. We let $\Gam^* =
    \Gam^{**} \cup \Gam'$ and $\Del^* = \Del^{**} \cup \Del' \cup (\al':B)$.
    We conclude since 
    \begin{itemize}
      \item $\Gam^* = \Gam^{**} \cup \Gam' \subseteq \Gam \cup \Gam'\cup \Gam'
      = \Gam \cup \Gam'$,  
      \item $\Del^* = \Del^{**} \cup \Del' \subseteq \Del \cup \Del' \cup
      (\al':B) \cup \Del' = \Del \cup \Del' \cup (\al':B)$.
    \end{itemize}
    
    \item $o=\termname{\beta}{t}$, where $\alpha \neq \beta$. Then
    $\replace{\alpha'}{\alpha}{s}{(\termname{\beta}{t})} =
    \termname{\beta}{\replace{\alpha'}{\alpha}{s}{t}}$. This holds by the \ih
    
    \item $o=\termrepl{\beta}{\gamma}{s'}{c}$, where $ \alpha \neq \beta$. Then
    $\replace{\alpha'}{\alpha}{s}{\termrepl{\beta}{\gamma}{s'}{c}} =
    \termrepl{\beta}{\gamma}{\replace{\alpha'}{\alpha}{s}{s'}}{\replace{\alpha'}{\alpha}{s}{c}}$.
    The typing derivation for $o$ has the following form: \[
    \Rule{\Gam_1  \vdash c \mid \Del_1, (\gamma : S' \tarrow B')^{\esta}, (\beta : B')^{\esta}, (\alpha : S \tarrow B)^{\esta}
          \quad
          \Gam'_1 \vdash s' \mid \Del'_1, (\beta : B')^{\esta}, (\alpha: S \tarrow B)^{\esta}
         }
         {\Gam_1 \cup \Gam'_1 \vdash \termrepl{\beta}{\gamma}{s'}{c} \mid \Del_1 \cup \Del'_1, \beta : B', (\alpha : S \tarrow B)^{\esta}}
         {} \]
    where $\Gam =\Gam_1 \cup \Gam'_1$ and $\Del = \Del_1 \cup \Del'_1,
    \beta : B', (\alpha : S \tarrow B)^{\esta}$.
    
    The \ih gives $\Gam^{**} \vdash \replace{\alpha'}{\alpha}{s}{c} \mid
    \Del^{**}$, where $\Gam^{**} \subseteq \Gam_1 \cup \Gam'$ and $\Del^{**}
    \subseteq (\Del_1, (\gamma : S' \tarrow B')^{\esta}) \cup \Del' \cup
    (\alpha' : B)$ as well as $\Gam^{***} \vdash
    \replace{\alpha'}{\alpha}{s}{s'} \mid \Del^{***}$, where $\Gam^{***}
    \subseteq \Gam'_1 \cup \Gam'$ and $\Del^{***} \subseteq \Del'_1 \cup \Del'
    \cup (\alpha':B)$. Then rule $(\trepl)$ gives $\Gam^{**} \cup \Gam^{***}
    \vdash \replace{\alpha'}{\alpha}{s}{c}\exrepl{\beta}{\gamma}{\replace{\alpha'}{\alpha}{s}{s'}}
    \mid (\Del^{**} \setminus (\gamma : S' \tarrow B')) \cup \Del^{***}, \beta
    : B'$. We conclude with
    \begin{itemize}
      \item $\Gam^{*} = \Gam^{**} \cup \Gam^{***} \subseteq (\Gam_1 \cup \Gam')
      \cup (\Gam'_1 \cup \Gam') = \Gam \cup \Gam'$ and
      \item $\Del^{*} = (\Del^{**} \setminus (\gamma : S' \tarrow B')) \cup
      \Del^{***} \cup (\beta:B') \subseteq \Del_1 \cup \Del' \cup (\alpha':B)
      \cup \Del'_1 \cup \Del' \cup (\alpha':B) \subseteq \Del \cup \Del' \cup
      (\alpha':B)$
  \end{itemize}
  
  \item $o=\termrepl{\alpha}{\gamma}{\termemst}{c}$. Then the typing derivation
  for $o$ has the following form: \[
  \Rule{\Gam \vdash c \mid \Del_1, (\gamma : \typeemst \tarrow  B')^{\esta}, (\alpha : S \tarrow B)^{\esta}
        \quad
        \emptyset \vdash \termemst: \typeemst  \mid \emptyset
       {\Gam \vdash \termrepl{\al}{\gamma}{\termemst}{c} \mid \Del_1, \al : S \tarrow B}
       {} \]
  where $\Del = \Del_1, \al: S \tarrow B$.

  The \ih gives $\Gam^{**} \vdash \replace{\alpha'}{\alpha}{s}{c} \mid
  \Del^{**}$, where $\Gam^{**} \subseteq \Gam \cup \Gam'$ and $\Del^{**}
  \subseteq (\Del_1, (\gamma : \typeemst \tarrow  B')^{\esta})\cup \Del' \cup
  (\alpha' : B)$.

  There are two cases to consider.
  \begin{enumerate}
    \item If $s \neq \termemst$. Then,
    $\replace{\alpha'}{\alpha}{s}{\termrepl{\alpha}{\gamma}{\termemst}{c}} =
    \termrepl{\alpha'}{\beta}{\termemst}{\termrepl{\beta}{\gamma}{s}{\replace{\alpha'}{\alpha}{s}{c}}}$
    and application of rule $(\trepl)$ gives $\Gam^{**} \cup \Gam' \vdash
    \replace{\alpha'}{\alpha}{s}{c}\exrepl{\beta}{\gamma}{s} \mid (\Del^{**}
    \setminus (\gamma : \typeemst \tarrow  B')) \cup \Del', \beta : B'$.
    Another application of rule $(\trepl)$ gives $\Gam^{**} \cup \Gam' \vdash
    \replace{\alpha'}{\alpha}{s}{c}\exrepl{\beta}{\gamma}{s}
    \exrepl{\al'}{\beta}{\termemst} \mid (((\Del^{**}\setminus (\gamma :
    \typeemst \tarrow  B')) \cup \Del') \setminus (\beta : B')), \al' : B$.
    We conclude with
    \begin{itemize}
      \item $\Gam^* = \Gam^{**} \cup \Gam' \subseteq \Gam \cup \Gam'$ 
      \item $\Del^* = (((\Del^{**} \setminus (\gamma : \typeemst \tarrow  B'))
      \cup \Del') \setminus (\beta:B')) \cup (\al':B) \subseteq \Del \cup \Del'
      \cup (\alpha':B)$
    \end{itemize}
    
    \item Otherwise (\ie $s = \termemst$),
    $\replace{\alpha'}{\alpha}{s}{\termrepl{\alpha}{\gamma}{\termemst}{c}}
    = \termrepl{\alpha'}{\gamma}{\termemst}{\replace{\alpha'}{\gamma}{s}{c}}$.
    Then application of rule $(\trepl)$ to $\Gam^{**} \vdash
    \replace{\alpha'}{\alpha}{s}{c} \mid \Del^{**}$ gives $\Gam^{**} \vdash
    \termrepl{\alpha'}{\gamma}{\termemst}{\replace{\alpha'}{\alpha}{s}{c}} \mid
    (\Del^{**} \setminus (\gamma : \typeemst \tarrow B')), \alpha':B'$. 
    We
    conclude with
    \begin{itemize}
      \item $\Gam^* = \Gam^{**} \subseteq \Gam \cup \Gam'$ 
      \item $\Del^* = (\Del^{**} \setminus (\gamma : \typeemst \tarrow B'))
      \cup (\alpha' : B') \subseteq (\Del_1 \setminus (\al : S \tarrow B)) \cup
      \Del' \cup (\al' : B) \subseteq \Del \cup \Del' \cup (\alpha' : B)$
    \end{itemize}
  \end{enumerate}
  
  \item $o = \termrepl{\alpha}{\gamma}{s'}{c}$, where $s' \neq \termemst$.
  Then, $\replace{\alpha'}{\alpha}{s}{\termrepl{\alpha}{\gamma}{s'}{c}} =
  \termrepl{\alpha'}{\gamma}{\termpush{\replace{\alpha'}{\alpha}{s}{s'}}{s}}{\replace{\alpha'}{\alpha}{s}{c}}$.
  Similar to the first case of explicit replacement.
\end{itemize}  
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> proofnets/bmc/ruleB1.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TS) {$\topnd{(\Gam, \Gam' \vdash \termapp{(\termabs{x}{t})}{u}:B \mid \Del, \Del')}$};
\node (N1) [below of=TS, yshift=-\PNdist] {$\toform{B}$};

\draw[PNarout] (TS.south) -- node{} (N1.north);
\end{tikzpicture}


==> proofnets/bmc/ruleB4.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TS) {$\topnd{(\Gam, \Gam'\vdash \termsubs{x}{u}{t}:B \mid \Del, \Del')}$};
\node (N1) [below of=TS, yshift=-\PNdist] {$\toform{B}$};

\draw[PNarout] (TS.south) -- node{} (N1.north);
\end{tikzpicture}


==> proofnets/bmc/ruleC1.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TS) {$\topnd{(\Gam, \Gam', \Gam'' \vdash \termrepl{\al'}{\al}{s}{\termrepl{\al}{\beta}{s'}{c}}:B \mid \Del, \Del', \Del'')}$};
\node (N1) [below of=TS, yshift=-\PNdist] {$\toform{B}$};

\draw[PNarrow] (TS.south) -- node[left]{$\alpha'$} (N1.north);
\end{tikzpicture}


==> proofnets/bmc/ruleC4.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TS) {$\topnd{(\Gam,\Gam',\Gam'' \vdash \termrepl{\al'}{\beta}{\termpush{s'}{s}}{c}:B \mid \Del,\Del',\Del'')}$};
\node (N1) [below of=TS, yshift=-\PNdist] {$\toform{B}$};

\draw[PNarrow] (TS.south) -- node[left]{$\alpha'$} (N1.north);
\end{tikzpicture}


==> proofnets/bmc/ruleM1.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TS) {$\topnd{(\Gam, \Gam' \vdash \termapp{(\termcont{\alpha}{c})}{u}:B \mid \Del, \Del')}$};
\node (N1) [below of=TS, yshift=-\PNdist] {$\toform{B}$};

\draw[PNarrow] (TS.south) -- node{} (N1.north);
\end{tikzpicture}


==> proofnets/bmc/ruleM3.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TS) {$\topnd{(\Gam, \Gam' \vdash \termcont{\alpha'}{\termrepl{\alpha'}{\alpha}{u}{c}} \mid \Del, \Del')}$};
\node (N1) [below of=TS, yshift=-\PNdist] {$\toform{B}$};

\draw[PNarrow] (TS.south) -- node{} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/lin1.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TR) {$\topnd{(\Gam, \Gam_1, \ldots, \Gam_n \vdash \termrepl{\alpha'}{\alpha}{s}{(\termname{\alpha}{u})} \mid \Del, \Del_1, \ldots, \Del_n, \alpha':B)}$};
\node (N1) [below of=TC, yshift=-\PNdist] {$\toform{B}$};

\draw[PNarrow] (TC.south) -- node[left]{$\alpha'$} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/lin5.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TN) {$\topnd{(\Gam, \Gam_1, \ldots, \Gam_n \vdash \termname{\alpha'}{\BMC{u \tconc s}} \mid \Del, \Del_1, \ldots, \Del_n, \alpha':B)}$};
\node (N1) [below of=TC, yshift=-\PNdist] {$\toform{B}$};

\draw[PNarrow] (TC.south) -- node[left]{$\alpha'$} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/rhoin1.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TC) {$\topnd{(\Gam \vdash \termname{\alpha}{\termcont{\beta}{c}} \mid \Del, \alpha: A)}$};
\node (N1) [below of=TC, yshift=-\PNdist] {$\toform{A}$};

\draw[PNarrow] (TC.south) -- node[left]{$\alpha$} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/rhoin5.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TC) [minimum width=\PNdist*4] {$\topnd{(\Gam \vdash c\exrepl{\alpha}{\beta}{\emst} \mid \Del, \alpha: A)}$};
\node (N1) [below of=TC, yshift=-\PNdist] {$\toform{A}$};

\draw[PNarrow] (TC.south) -- node[left]{$\alpha$} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/rhonotin1.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TC) {$\topnd{(\Gam \vdash \termname{\alpha}{\termcont{\beta}{c}} \mid \Del, \alpha: A)}$};
\node (N1) [below of=TC, yshift=-\PNdist] {$\toform{A}$};

\draw[PNarrow] (TC.south) -- node[left]{$\alpha$} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/rhonotin5.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TC) [minimum width=\PNdist*4] {$\topnd{(\Gam \vdash c\exrepl{\alpha}{\beta}{\emst} \mid \Del, \alpha: A)}$};
\node (N1) [below of=TC, yshift=-\PNdist] {$\toform{A}$};

\draw[PNarrow] (TC.south) -- node[left]{$\alpha$} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/ttabs1.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TS) {$\topnd{(\Gam, \Gam' \vdash \termsubs{x}{u}{(\termabs{y}{v})}:\typefunc{A_y}{B} \mid \Del, \Del')}$};
\node (N1) [below of=TS, yshift=-\PNdist] {$\toform{(\typefunc{A_y}{B})}$};

\draw[PNarout] (TS.south) -- node{} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/ttabs3.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TA) {$\topnd{(\Gam, \Gam' \vdash \termabs{y}{\termsubs{x}{u}{v}}:\typefunc{A_y}{B} \mid \Del, \Del')}$};
\node (N1) [below of=TA, yshift=-\PNdist] {$\toform{(\typefunc{A_y}{B})}$};

\draw[PNarout] (TA.south) -- node{} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/ttapp1.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TS) {$\topnd{(\Gam, \Gam', \Gam'' \vdash \termsubs{x}{u}{(\termapp{v}{r})}:B \mid \Del, \Del', \Del'')}$};
\node (N1) [below of=TS, yshift=-\PNdist] {$\toform{B}$};

\draw[PNarout] (TS.south) -- node{} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/ttapp3.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TA) {$\topnd{(\Gam, \Gam', \Gam'' \vdash \termapp{\termsubs{x}{u}{v}}{r}:B \mid \Del, \Del', \Del'')}$};
\node (N1) [below of=TA, yshift=-\PNdist] {$\toform{B}$};

\draw[PNarout] (TA.south) -- node{} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/ttname1.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TS) {$\topnd{(\Gam, \Gam' \vdash \termsubs{x}{u}{(\termcont{\alpha}{\termname{\beta}{v}})}:A \mid \Del, \Del')}$};
\node (N1) [below of=TS, yshift=-\PNdist] {$\toform{A}$};

\draw[PNarout] (TS.south) -- node{} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/ttname3.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TN) {$\topnd{(\Gam, \Gam' \vdash \termcont{\alpha}{\termname{\beta}{\termsubs{x}{u}{v}}}:A \mid \Del, \Del')}$};
\node (N1) [below of=TN, yshift=-\PNdist] {$\toform{A}$};

\draw[PNarout] (TN.south) -- node{} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/ttrepl1.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TS) {$\topnd{(\Gam, \Gam', \Gam'' \vdash \termsubs{x}{u}{(\termcont{\alpha}{\termrepl{\beta'}{\beta}{s}{\ctxtapp{\ctxtLCT'}{v}}})}:A \mid \Del, \Del', \Del'', \beta':B)}$};
\node (N1) [below of=TS, yshift=-\PNdist] {$\toform{A}$};

\draw[PNarout] (TS.south) -- node{} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/ttrepl6.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TC) {$\topnd{(\Gam, \Gam', \Gam'' \vdash \termcont{\alpha}{\termrepl{\beta'}{\beta}{s}{\ctxtapp{\ctxtLCT'}{\termsubs{x}{u}{v}}}}:A \mid \Del, \Del', \Del'', \beta':B)}$};
\node (N1) [below of=TC, yshift=-\PNdist] {$\toform{A}$};

\draw[PNarout] (TC.south) -- node{} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/ttsub1.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TS) {$\topnd{(\Gam, \Gam', \Gam'' \vdash \termsubs{x}{u}{\termsubs{y}{r}{v}}:B \mid \Del, \Del', \Del'')}$};
\node (N1) [below of=TS, yshift=-\PNdist] {$\toform{B}$};

\draw[PNarout] (TS.south) -- node{} (N1.north);
\end{tikzpicture}


==> proofnets/soundness/ttsub3.tex <==
\begin{tikzpicture}[baseline=(current bounding box.center),node distance=\PNdist]
\node[PNsub] (TS) {$\topnd{(\Gam, \Gam', \Gam'' \vdash \termsubs{y}{r}{\termsubs{x}{u}{v}}:B \mid \Del, \Del', \Del'')}$};
\node (N1) [below of=TS, yshift=-\PNdist] {$\toform{B}$};

\draw[PNarout] (TS.south) -- node{} (N1.north);
\end{tikzpicture}

